Fractional-gradient Sparsity with Autoencoding Sequential Deep Image Prior for 3D CT Reconstruction

3D volumetric reconstruction from incomplete or noisy measurements is a fundamental problem in medical imaging and computational tomography. Deep image prior (DIP)-based methods have recently shown strong capability for solving inverse problems without requiring large training datasets. However, directly extending DIP to 3D reconstruction by fully 3D networks can incur high computational cost, while slice-by-slice 2D DIP approaches may lead to inter-slice inconsistencies due to the lack of explicit regularization along the third direction. In this paper, we propose a novel volumetric reconstruction framework, Fractional-gradient Autoencoding Sequential Tomography DIP (FAST-DIP), which integrates input-adaptive sequential deep image prior modeling of slices with fractional sparsity regularization to capture inter-slice dependencies. Specifically, we introduce a fractional l1/l2-based sparsity prior on the gradients along the slice (z) direction to explicitly enforce inter-slice structural consistency. We further provide theoretical analysis of the proposed alternating minimization algorithm under the majorization-minimization (MM) framework, establishing monotonic descent of the objective function and convergence to a critical point under the Kurdyka-Lojasiewicz (KL) property. Experimental results for 3D X-ray computed tomography (CT) reconstruction demonstrate that the proposed method improved reconstruction quality and structural consistency compared with existing DIP-based approaches.

==> sec/2_related.tex <==
\section{Related Works}
\label{sec:related}

\subsection{ASeqDIP}

The Autoencoding Sequential Deep Image Prior (ASeqDIP) \cite{alkhouri2024image} extends the classical Deep Image Prior (DIP) \cite{ulyanov2018deep} framework by incorporating sequential input adaptation during reconstruction. Consider an inverse imaging problem where the observation $\textbf{y} \in \mathbb{R}^m$ is generated through a forward operator $\textbf{A}$ as:
\begin{equation}
\textbf{y} = \textbf{A} \textbf{x} + \textbf{n},
\end{equation}
where $\textbf{x} \in \mathbb{R}^n$ (discretized) denotes the unknown clean image and $\textbf{n}$ represents measurement noise. 
In the original DIP formulation, the reconstruction is produced by a randomly initialized neural network $f_{\phi}(\cdot)$ that maps a fixed random input $\textbf{z}$ to an image estimate. The network parameters are optimized by minimizing a data consistency objective:
\begin{equation}
\min_{\phi} \; \| \mathbf{A}f_{\phi}\mathbf{(z)} - \mathbf{y} \|_2^2.
\end{equation}

Recent work has shown that while DIP provides a strong implicit prior, its optimization can become unstable and overfit measurement noise \cite{liang2025analysis}, motivating additional regularization and stabilization strategies \cite{cheng2019bayesian,wang2023early}. 
%Related approaches such as DeepRED explicitly combine DIP with denoiser-based regularization to improve reconstruction robustness \cite{mataev2019deepred}; ASeqDIP follows this direction by introducing an autoencoding constraint together with sequential input refinement.
ASeqDIP \cite{alkhouri2024image} used an autoencoding constraint together with sequential input refinement to improve the DIP method.
%The ASeqDIP modifies this paradigm by 
It introduced a sequence of progressively refined inputs. In stage $t$, the network generates an intermediate reconstruction $f_{\phi}(\mathbf{z}_t)$ 
%\begin{equation}
%\mathbf{x}_t = f_{\phi}(\mathbf{z}_t),
%\end{equation}
and the optimization objective becomes:
\begin{equation}
\min_{\phi}
\|\textbf{A} f_{\phi}(\textbf{z}_t)- \textbf{y}\|_2^2
+
\lambda \|f_{\phi}(\textbf{z}_t) - \textbf{z}_t\|_2^2.
\end{equation}
The additional autoencoding regularization term encourages the output to remain close to its input, preventing unstable updates while guiding the reconstruction toward measurement-consistent structures.
After each stage, the output (with refined network) is used to update the next input as:
\begin{equation}
\mathbf{z}_{t+1} = \textbf{x}_t = f_{\phi}(\mathbf{z}_t). 
\end{equation}
Changing between network optimization and input refinement, ASeqDIP produces a sequence of progressively improved or denoised reconstructions. This sequential strategy helps mitigate the overfitting behavior commonly observed in standard DIP optimization \cite{wang2021early}.


\subsection{Fractional-Gradient Sparsity Prior}
% from the sparsity: 
Sparsity-promoting regularization plays an important role in inverse imaging problems. Classical approaches such as $\ell_1$ regularization and total variation (TV) enforce the sparsity of image gradients and have been widely used for image reconstruction tasks \cite{ritschl2011improved,huang2024edge,wu2024medical}. In particular, the TV seminorm can be interpreted as the $\ell_1$ norm of the image gradient \cite{wang2022minimizing}. It is well known that the $\ell_1$ norm serves as the tightest convex relaxation of the $\ell_0$ norm, which directly measures sparsity of signals. However, TV-based regularization is sensitive to the scale of gradients and may introduce staircase artifacts when modeling piecewise-smooth structures \cite{jiang2023inexact}.

To better approximate the $\ell_0$ norm, several alternative sparsity-promoting regularizations have been proposed, including nonconvex $\ell_p$ penalties with $0<p<1$ \cite{wu2021two} and fractional sparsity formulations such as the $\ell_1/\ell_2$ ratio \cite{wang2022minimizing}. In particular, the $\ell_1/\ell_2$ regularization has been shown to effectively mitigate the staircasing artifacts commonly produced by TV, since the $\ell_2$ norm of the gradient in the denominator discourages trivial shrinkage of the entire gradient field \cite{wang2021limited}. Moreover, the $\ell_1/\ell_2$ penalty promotes structured sparsity by encouraging many gradient components to approach zero while preserving the relative magnitude of significant gradients. Due to its scale-invariant property, this type of regularization has demonstrated advantages in various inverse problems, including compressed sensing and image restoration.

Motivated by these observations, we adopt a fractional-gradient sparsity prior to model sparse variations along the slice direction in volumetric reconstruction. The proposed regularization focuses on the sparsity of inter-slice gradients, which helps preserve intra-slice structural details while enforcing structural consistency across neighboring slices.




==> sec/7_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
